Augmenting Sports Videos with VisCommentator

Visualizing data in sports videos is gaining traction in sports analytics, given its ability to communicate insights and explicate player strategies engagingly. However, augmenting sports videos with such data visualizations is challenging, especially for sports analysts, as it requires considerable expertise in video editing. To ease the creation process, we present a design space that characterizes augmented sports videos at an element-level (what the constituents are) and clip-level (how those constituents are organized). We do so by systematically reviewing 233 examples of augmented sports videos collected from TV channels, teams, and leagues. The design space guides selection of data insights and visualizations for various purposes. Informed by the design space and close collaboration with domain experts, we design VisCommentator, a fast prototyping tool, to eases the creation of augmented table tennis videos by leveraging machine learning-based data extractors and design space-based visualization recommendations. With VisCommentator, sports analysts can create an augmented video by selecting the data to visualize instead of manually drawing the graphical marks. Our system can be generalized to other racket sports (e.g., tennis, badminton) once the underlying datasets and models are available. A user study with seven domain experts shows high satisfaction with our system, confirms that the participants can reproduce augmented sports videos in a short period, and provides insightful implications into future improvements and opportunities.

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS, incl. InfoVis, SciVis, VAST)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> tex/_deprecated/1-intro.tex <==
\firstsection{Introduction}
\maketitle

%% why, who, when need augmented videos
Video is a popular form to present and broadcast sports events.
In recent years,
thanks to the advance of techniques such as Computer Vision (CV) and Image Processing (IP),
there has been a growing practice of augmenting sports videos with embedded visualizations~\cite{fischer2019video}.
These augmented sports videos combine visualizations
with video effects (\emph{e.g.}, slow motion, and camera rotation)
to embed the data in the actual scenes (\emph{e.g.}, \autoref{fig:teaser}Right).
Given the ability to explicate player strategies in an engaging manner,
augmented sports videos have been widely used by TV channels~\cite{espn} to engage the fans
and sports analysts~\cite{perin2018state, stein2017bring} to communicate analytical findings.

% TV channels~\cite{espn}, sports teams~\cite{celtics},
% to inform the fans
% and sports teams~\cite{celtics} to engage or inform the audiences.

%% current practices, follow
%% the specific challenges different from other storytellings
Despite their popularity,
these augmented videos, by nature, are difficult to create,
especially for sports analysts, who
usually lack sufficient video editing skills compared to the proficient video creators in TV companies.
Based on our collaboration with sports analysts
who provide data analysis and consultancy services for national sports teams,
we are informed that augmenting videos are particularly useful for the sports analysts,
allowing them to effectively communicate the analytical insights to the coaching team and players.
However, the sports analysts usually are unable to create these videos,
as the creation process involves many design decisions and complex video editing.
Thus, fast prototyping tools that allow sports analysts to create augmented videos rapidly
are in great demand.

% Usually, these videos cannot be created without sports experts.
% we identify that the typical workflow to create augmented sports videos
% mainly includes two steps:
% 1) analyze a sports video to obtain data insights;
% and 2) edit and augment the video with these data insights.

% We are also informed that these two steps are usually finished by sports experts---even in some cases (\emph{e.g.}, for TV channels) the final video can be created by video editors, 
% sports experts still need to prototype a video or sketch to communicate the insights.
% 
% leading to a high entry barrier to sports video augmentation.

%% SOTA
Various systems and techniques have been proposed 
to augment sports video over the last years.
On the one hand,
industrial companies have developed commercial tools, 
such as Viz Libero~\cite{vizrt} and Piero~\cite{piero}, for TV sportscast.
% Although these tools provide powerful video editing functions,
% they 
Yet, these tools target at proficient video editors (\emph{e.g.}, who work at TV companies)
and have a steep learning curve.
On the other hand,
although an increasing research
has been conducted on sports data visualization,
visualizing data in sports videos has received relatively less attention from the community~\cite{perin2018state}.
A notable exception comes from Stein et al.~\cite{stein2017bring, stein2018},
who developed a system that 
automatically extracts and visualizes data from and in \emph{soccer} videos.
Nonetheless, except for soccer, there are no publicly available methodologies and tools
that help sports analysts create augmented sports videos 
by providing data-driven features (\emph{e.g.}, visualizations recommendation, mapping and binding between data and visuals).

Similar to all data visualizations,
the creation of augmented sports videos 
can be divided into two stages, namely, data analysis and visualization.
To facilitate the creation of augmented sports videos,
we are particularly interested in four questions that should be considered
in the two stages:
1) In the data analysis stage,
\emph{what kinds of data can be used to augment a sports video (Q1)?}
Among all the available data, % that is available for augmenting a sports video,
\emph{what data should be presented regarding to various narrative purposes (Q2)?};
2) In the visualization stage,
\emph{what visual effects are used to present these data (Q3)?}
\emph{How to organize these visual effects in temporal order with respect to the raw video (Q4)?}
From a tool-design perspective,
these questions can also be reorganized into 
\emph{element-level} (Q1, Q3),
which are about the building blocks for augmenting sports videos,
and \emph{clip-level} (Q2, Q4),
which are about the the organization of these building blocks.
Without understanding these questions,
the visualizations embedded in the fast-moving sports video will easily overwhelm the audience, let alone to engage them.

In this work, 
we focus on ball sports and aim to facilitate the creation of augmented videos for sports experts.
% We first contribute a design space by
% systematically reviewing \numVideo{} examples
% collected from reputable sources (\emph{e.g.}, TV channels, leagues, and teams).
% to understand the design practices of augmented videos.
To understand the design practices of augmented sports videos,
we first systematically reviewed a corpus of \numVideo{} examples
collected from reputable sources (\emph{e.g.}, TV channels, leagues, and teams). 
Our analysis resulted in a design space that characterizes augmented sports videos at element- and clip-levels,
which answer the aforementioned four questions.
% we first contribute a design space 
% derived from a systematic review of \numVideo{} examples 
% collected from reputable sources (\emph{e.g.}, TV channels, leagues, and teams).
% Our analysis resulted in a 
% The design space characterizes augmented sports videos at element- and clip-levels,
% which answers the aforementioned four questions.
The four design dimensions (\emph{i.e.}, \DT{}, \DV{}, \DD{}, and \DN{}) of the design space
and their combination frequency
provide guidance for selecting data insights and visual effects for various purposes (\emph{i.e.}, engagement or education).
Informed by the design space, 
we design and implement \system{},
a proof-of-concept system that facilitates the creation of augmented table tennis videos.
\system{} takes a raw table tennis video as the input,
extracts analytical data,
and semi-automatically suggests visual effects 
% recommendation engine
% features two recommendation engines
% to 
based on the narrative purpose, narrative order, and augmented data selected by the user.
Integrated with existing video editors,
\system{} allows sports experts to fast prototype augmented table tennis videos.
Due to the data-driven nature, \system{} can be generalized to other turn-taking ball games such as
tennis and badminton once data and the underline models are available.
%% evaluation
\cmo{evaluation}
% A user study with seven sports experts confirms 
% the utility and usability of the system. 
% A group of 23 sports fans found the augmented videos created by the experts informative and engaging.
% We further report the experts’ feedback gathered from the post-study interviews,
% which implies future improvements and opportunities.
The corpus, created videos, and other materials can be found in \url{https://viscommentator.github.io} (clean and safe).


==> tex/_deprecated/2-related.tex <==
\section{Related Work}

\subsection{Video-based Sports Visualization}
Due to its advantages of presenting data in actual scenes,
video-based sports visualization has been widely used to
ease experts' analysis~\cite{stein2017bring} 
and engage the audiences~\cite{lin2020sportsxr}.
Based on the presentation method, 
video-based visualizations
can be divided into side-by-side~\cite{Zhi2019},
overlaid~\cite{tang2020design} (\emph{i.e.},),
and embedded~\cite{stein2017bring} (\emph{i.e.},).
% two types, \emph{i.e.}, overlaid and embedded.
This work focuses on embedded visualizations in sports videos.

Perin et al.~\cite{perin2018state} 
comprehensively surveyed the visualization research on sports data,
indicating that only a few works can be considered as video-based visualizations.
Among these few works,
a representative example were developed by Stein et al.~\cite{stein2017bring} for soccer.
Their system takes a raw footage as the input 
and automatically visualizes some tactical information as graphical marks in the video.
Later, Stein et al.~\cite{stein2018} extended their work 
by proposing a conceptual framework that semi-automatically
select proper information to be presented at a given moment.
Recently, 
Fischer et al.~\cite{fischer2019video} found that video-based soccer visualization systems from industry are actually ahead of most of the academic research.
For example, 
Piero~\cite{piero} and Viz Libero~\cite{vizrt} are both developed for sportscasting
and provide a set of powerful functions to edit and annotate a sports video.
Besides, CourtVision~\cite{courtvision}, developed by Second Spectrum~\cite{secondspectrum} for basketball, 
is another industry product that automatically tracks players positions 
and embeds status information to engage the audiences.
In summary, as detailed by Fischer et al.~\cite{fischer2019video},
the research on video-based sports visualization is still in its infancy, 
while the strong market demand has already spawned very successful commercial systems.
Nevertheless, 
these commercial systems target at proficient video editors,
% and provide comprehensive video editing features,
leading to a steep learning curve for sports analysts.
Moreover, they %rarely enable data-driven designs whereas
mainly augment the video with graphical elements,
while the goal of sports analysts is to augment sports videos with data.
% enable data-driven design which plays an important role
% in creating augmented sports videos.
Given that very little is known about the design practices of augmented sports videos, 
it remains unclear how to support augmenting sports videos with data.
% what data-driven features should be provided to facilitate their creation.
In this work, we explore this direction and aim to ease the creation
by a systematic study of existing augmented sports videos collected
from reputable sources.

\subsection{Data Videos for Storytelling}
%% What is Data-driven storytelling
% Data-driven storytelling, also known as Narrative Visualization,
% studies the ways to visually communicate data insights.
Data video, 
as one of the seven genres of narrative visualization categorized by
Segel and Heer~\cite{narrativeVis},
% categorized narrative visualization into seven genres.
% As one of these seven genres, 
is an active research topic and has attracted interest from researchers.
Amini et al.~\cite{amini2015} systematically analyzed 50 data videos from reputable sources and summarized the most common visual elements and attention cues in these videos.
They further deconstructed each video into four narrative categories
by using the visual narrative structure theory introduced by Cohn~\cite{cohn2013}.
Their findings reveal some design patterns in data videos 
and provide implications for the design of data video authoring tools.
Build upon of that, Amini et al.~\cite{Amini2017} further contributed DataClips,
an authoring tool that allows general users to craft data videos with predefined templates.
Recently, 
Thompson et al.~\cite{Thompson2020} contributed a design space of data videos
for developing future animated data graphic authoring tools.
Cao et al.~\cite{cao2020} analyzed 70 data videos and proposed a taxonomy to
% contributed two design spaces of data videos 
characterize narrative constructs in data videos.

%% Embedded
Although these studies provide insights into data videos design,
our scenario is inherently different from theirs and thus yields new challenges.
Specifically,
these studies use video as a medium to tell the story of data,
whereas we focus on augmenting existing videos with data.
An existing video imposes extra constraints 
on narrative orders, data visual forms, \emph{etc.}
With these constraints,
how to visually narrate data in videos remains underexplored.
Perhaps the most relevant work is from Stein et al.~\cite{stein2018},
who annotated the data in soccer videos in a linear way.
To fully explore the ways for augmenting sports videos with data,
% the narrative orders used 
% for presenting data in augmented sports videos,
we analyze \numVideo{} real-world examples 
and summarize six narrative orders and their common usage scenarios.
% These analyzed 
The results provide guidance for designing 
authoring tools of augmented sports videos.

\subsection{Intelligent Design Tools}
Designing visual data stories usually requires the skills to analyze complex data 
and map it into proper visualizations,
both of which require considerable skills.
Therefore, to lower the enter barrier to visual data stories,
many researchers develop intelligent creation tools 
to automate or semi-automate the design process.
To ease the visual mapping process,
one widely used approach is templates. 
For example,
DataClips~\cite{Amini2017} and Timeline StoryTeller~\cite{brehmer2017} use templates manually summarized from existing examples to enable semi-automatic creation of data animation and timeline infographics, respectively.
On the basis of Timeline StoryTeller, Chen et al.~\cite{chentimeline} proposed a method to automatically extract extensible templates from existing designs
to automate the timeline infographics design.
Besides automating the visual mapping process,
some tools further facilitate the data analysis process 
by automatically suggesting data insights.
%% Data-shot
DataShot~\cite{WangSZCXMZ20} adopts an auto-insight technique to recommend interesting data insights based on their significance for factsheet generation.
%% Data-toon
DataToon~\cite{kim2020}, an authoring tool for data comic creation, 
uses a pattern detection engine 
to automatically suggest interesting patterns of the input network data.

However, few, if any, tools exist that provide the aforementioned kinds of
data-driven support for creating augmented sports videos.
The challenges of developing such a tool not only exist 
in the engineering implementations but also in the integration
between the workflows of visualization authoring and video editing.
We draw on the line with prior visualization design tools
and design \system{} to support visualizing data in sports videos
in a common video editing workflow.

\subsection{Data Extraction from Sports Videos}
Due to the advancement of deep learning on CV,
such as object detection~\cite{Ren2015}, segmentation~\cite{Redmon2015}, 
and action recognition~\cite{zhang2019pan}, 
more and more data is available to be extracted from a sports video.
Shih~\cite{shih2017survey} 
presented a comprehensive survey on content-aware video analysis for sports.
He summarized the state-of-the-art techniques to parse sports videos
from a low-semantic to a high-semantic level:
1) object level techniques extract the key objects in the video, 
2) event level recognizes the action of the key object, 
and 3) conclusion level generates the semantic summarization of the video.
% object detection and action recognition~\cite{},
% highlight detection and event recognition~\cite{}, 
% and contextual inference and semantic analysis~\cite{}
% (\emph{e.g.}, event outcomes and match summaries).
Besides models tailored to sports videos,
researchers have also developed models~\cite{nguyen2016} to detect and segment human from images and videos in general scenarios.
A particular challenge in table tennis is that
the ball is small (\emph{e.g.}, 15 pixels on average~\cite{ttnet}) 
and move fast (\emph{e.g.}, $30$ $m/s$).
To tackle this challenge, Voeikov et al.~\cite{ttnet}
proposed TTNet, a convolution-based neural network,
that detects the ball in a high-resolution video.
Besides, TTNet can further segments the ball 
and detect ball events such as bounces and net hits.
In this work,
we composite multiple state-of-the-art machine learning models~\cite{ttnet, bodypiex2, he2016}
to extract the data from table tennis videos with a fixed camera angle,
such as ball and players position, actions, events, and key strokes.

%% stroke action classification
% Besides detecting the ball, Martin et al.~\cite{}
% introduced 

% Fine grained action classification has raised new challenges compared to classical action classification problem. Sport video analysis
% is a very popular research topic, due to the variety of application areas, ranging from multimedia intelligent devices with user-tailored
% digests, up to analysis of athletes’ performances. Running since 2019
% as a part of MediaEval, we offer a task which consists in classifying
% table tennis strokes from videos recorded in natural conditions at
% the University of Bordeaux. The aim is to build tools for teachers,
% coaches and players to analyse table tennis games. Such tools could
% lead to an automatic profiling of the player and the training session
% could then be adapted for improving sports skills more efficiently.

==> tex/_deprecated/4-system.tex <==
% \clearpage
% \setlength{\intextsep}{12.0pt plus 2.0pt minus 2.0pt}

\section{\system{}}
Based on the design space,
we design \system{}, 
a proof-of-concept that 
% facilitates the creation of augmented sports videos for table tennis.
augments the videos for table tennis.
While the implementation of \system{} is specific to table tennis, 
its design can be generalized to other racket ball sports (\emph{e.g.}, tennis, badminton)
once the underlying dataset and ML models are available.

\subsection{Design Goals}
We conceived the design goals of \system{} 
based on the design space, 
prior research~\cite{WangSZCXMZ20, kim2020, shicalliope} on intelligent data visualization design tools,
and weekly meetings with two domain experts over the past eleven months.
One of the experts is a sports science professor, who
provides data analysis and consultancy services for national table tennis teams.
The other is a Ph.D. candidate in sports science with a focus on table tennis analytics.
In the meetings, we 
% proactively communicated with the experts, 
demonstrated several prototype systems
and collected feedback to refine our design goals.

% \noindent
% \textbf{\cmo{G1. Integrated with General Video Editing Tools.}}
% Augmented sports videos are produced by augmenting
% raw sports videos with data.
% Besides the data augmentations,
% there are many editing on the video (\emph{e.g.}, slice a clip, compress the video) 
% can and should be finished by general video editing tools.
% Therefore, instead of being a separated authoring tool,
% the system to create augmented videos should be able to be integrated into a general video editing tool.

\textbf{G1. Extract the Data from the Video based on Data Levels.}
The analyst may augment the video with different data for different purposes.
Based on our design space, augmented sports videos usually present data from different levels
for entertainment or education purposes.
Thus,
to support these augmentations, % and reduce the analyst's workload, 
the system should automatically extract the data from different levels,
namely, object-, event-, and tactic-levels.
\cmo{Besides, the data should be organized in a hierarchical manner according to the data level
for efficiently accessing.}

%  the analyst may augment the video fordifferent purposes. 
%  To support these augmentation, VisCommentatorneeds to obtain the data from different levels, namely, . We implement a bottom-up approach toextract the data from table tennis videos. The user can also import thedata from other tools [].

% \noindent
% \textbf{G2. Recommend Data Insights for Different Purposes.}
% Many intelligent data design tools~\cite{WangSZCXMZ20, shicalliope} adopt auto-insights techniques to
% alleviate the data analysis burden by automatically suggesting interesting data patterns.
% However, as described in Sec.~\ref{ssec:design_clip}, 
% augmented videos 
% present different data for different narrative purposes (\emph{e.g.}, engaging or education).
% Thus,
% we intend that the system should recommend data insights 
% based on the user's narrative purposes.

\textbf{G2. Augment the Video with Data Instead of Graphical Marks.}
The fundamental goal of sports analysts is to \emph{visualize a data}, 
\emph{e.g.}, show the ball trajectory. 
However, most of the commercial video editing tools ask the user to \emph{select a graphical mark}
to augment the raw footage, \emph{e.g.}, draw a line in the scene.
Hence, the system should allow the analysts
to select the data to be visualized instead of asking them to select the graphical mark to draw. 

% \noindent
\textbf{G3. Recommend Visualizations for Different Narrative Orders.}
Visualization recommendation systems can ease the creation process as the sports analysts may lack sufficient
knowledge of data visualization.
Prior systems~\cite{voyager, draco} usually recommend  visualizations
based on the effectiveness of visual channels.
However, in our scenarios, 
the narrative order that may result in different availability of visual effects.
For example, when using a \DNL{} order, we cannot move a player in the video out of his position.
Consequently, the system should further consider the narrative order
in the recommendation.

\begin{figure*}[hbt]
  \centering
  \includegraphics[width=0.99\textwidth]{figs/4_ui.jpg}
  \caption{
    a)-c) The user interface of the system, including a video preview, a main timeline,
    and an edit panel.
    d) The rotation speed of the ball is 7000 rotation per minute.
    e) The probability distribution of the ball placement on the table.
    f) The player attacks the ball to win the rally.
    g) The video uses a \DNFF{} order to preview the action of the player after showing the potential ball placement.
  }
 \label{fig:ui}
\end{figure*}


\subsection{Usage Scenario}
To illustrate how \system{} encompasses the design goals,
% and the key user interfaces (UIs), 
we introduce the workflow to create an augmented video taken by Jon,
a hypothetical sports analyst
who needs to analyze a table tennis rally
and present his findings to the coaching team and athletes.
He also needs to create a video with highlight moments to engage the team fans.

\para{Brush to focus.}
To create the augmented video, Jon loads the raw video to \system{}.
Jon is familiar with the UI of \system{} 
as it follows the design of general video editing tools (G1),
which usually have a video preview (\autoref{fig:ui}a),
a main video timeline to be edited (\autoref{fig:ui}b),
and an edit panel in the right-hand side (\autoref{fig:ui}c).
The loaded video file appears in the main timeline.
Each turn of the rally is automatically detected and visualized under the timeline.
After analyzing the video,
Jon notices that the last second turn is the key movement,
in which the ball rotation speed
is so fast that the player in red cloth ($Player_{red}$)
can only return it to a narrow area
and thus gives his opponent a chance to attack.
Hence, Jon brushes on the timeline to select the last two turns to augment the video. 
% to augment this moment.
% which he thinks is the highlight moment of the rally.

\para{Select to augment.}
An edit panel titled ``How to augment this clip?'' is opened in the right (\autoref{fig:ui}c).
In the panel, there are two button groups, 
``Narrative Purpose'' and ``Narrative Order'',
with \emph{Education} and \emph{Linear} in default, respectively.
The bottom is a list that shows the visual mappings (\autoref{fig:ui}c1). %%``Visual Mapping'' list.
% with some pre-selected data-visual mappings.
%% in the video, the player and ball is highlighted by bbox
%% right click the ball, to select the data
%% right click the player to select 
%% auto augmentation
The two players and ball are automatically detected and highlighted 
by using bounding boxes in the main view (\autoref{fig:ui}a).
A context menu popups when Jon right-clicks the players or ball, 
allowing Jon to directly select which data to be augmented (\autoref{fig:ui}a1, G2).
Jon first moves the pointer to the frame when $Player_{red}$ perform the stroke (\autoref{fig:ui}b1)
and right-clicks the ball in the main view.
% showing a list of ball data, 
% such as ``Potential placements'', ``Potential routes'', and ``Trajectory'',
% By switching different ``Narrative Purpose'',
% Jon notices that the available data options in the context menu change accordingly.
% By hovering on the \emph{Education} option,
% Jon is informed that this option allows augmenting the video with tactical data.
Based on his analysis,
% Jon wants to highlight 
% that 
% the player in red cloth cannot perform a high-quality return is because
% the ball rotation speed is so fast that the player can only return it to a narrow area.
% Thus, 
Jon selects the ``Ball rotation speed'', ``Potential placements'', and ``Potential routes''
% which he thinks to be the key data that reveal the failure of the player in  red cloth,
in the context menu.
The system automatically recommends visual effects for these data 
and lists the mappings in the ``Visual Mapping'' list (G3).
Interested in how the augmentation looks like, 
Jon plays the video and finds out that the video is augmented by visualizations.
The augmented clip pauses and visualizes 
the ball rotation speed by using a label (\autoref{fig:ui}d),
followed by an animation that shows 
the potential routes and placements possibility of the ball (\autoref{fig:ui}e).
Satisfied with these augmentation,
Jon moves the pointer to the next turn,
right-clicks the player in black cloth ($Player_{black}$),
and selects the ``Stroke Technique'' data.
Consequently, \system{} augments the video to highlight the active attack of $Player_{black}$ (\autoref{fig:ui}f).
% when performs the 
% This obviously gives a chance to his opponent, who performs an active attack (\autoref{fig:ui}f)
% in the next move and successfully win the game.
% Besides,
% the system previews a clip augmented by visualizations in the main view.
% to explain why the player wins the rally.
% Jon selects 
% which he thinks are the key data that reflects the 
% Jon clicks the ``Generate'' button at the bottom of the edit panel.
% The augmented clip reveals that the rotation speed of the ball
% is so fast (\autoref{fig:ui}d) that the player in red cloth
% can only return it to a narrow area 
%% another effect with the same data
Although impressed with these augmentations, 
Jon is curious about the ``Narrative Order''and chooses ``Flash Forward'' 
to check the augmentation effects.
The system presents another augmented clip that
foreshadows the action of the opponent in the video
right after showing the probability distributions of the ball placement
(\autoref{fig:ui}g).
Jon recognizes that this narrative method 
explains the causality between the ball placement and the opponent's attack in a stronger manner. 

% \vspace{-1mm}
\para{Edit and Fine-tune.}
Besides the coaching team and athletes, 
Jon also needs to present the highlight moments to engage the team fans.
Jon thinks that the tactical data is too complex for the general fans.
% given that the target audiences may have little knowledge of table tennis, 
% Jon thinks that the tactical data is too complex for them.
%% choose another batch of data
Consequently, Jon chooses \emph{Engagement} for the ``Narrative Purpose'',
which allows him to augment the video with physical data.
Instead of annotating the key players' movements,
the resulting augmentation highlights the ball trace with slow motion (\autoref{fig:ui}a),
which Jon believes will be favored by the audiences.
He further selects three more physical data (\emph{i.e.},
``Player Position'', ``Player Trajectory'', and ``Ball Placement") 
in the ``Visual Mapping'' list to augment the clip.
\system{} automatically recommends visual effects to present these data, 
so that Jon only needs to perform minimal editions, \emph{e.g.}, specify the colors.
Satisfied with the results, Jon exports the augmented video.

\begin{figure*}[th]
  \centering
  \includegraphics[width=\textwidth]{figs/4_pipeline5.jpg}
  \caption{The pipeline to augment a raw footage. a) The input video. b) The extracted data is organized into a data pyramid. 
  c) After selecting a level of data and brushing a specific period, 
  the system returns a subtree and automatically suggests interesting data insights, \emph{e.g.}, the two events in cyan.
  d) The system constructs a Directed Acyclic Graph based on the user-selected
  narrative orders and suggests visual mappings for each data nodes.
  f) Rendering and generating the augmented video. }
 \label{fig:pipeline}
\end{figure*}

\input{tex/43-data-processing}
\input{tex/44-userinteraction}
\input{tex/45-visualization}

\begin{figure*}[h]
  \centering
  \includegraphics[width=\textwidth]{figs/62_case.jpg}
  \caption{
    a)-d) An \DNFF{} augmented video example created by an expert:
    a) The augmentation shows that when the player in black plans to move to the right,
    his opponent attempts to stroke the ball to the left.
    b) The player in black tries his best to return the ball.
    c) After he return the ball, his opponent strokes the ball to the right, d) which is too far away for him to return the ball. Thus, he loses this rally.
    e)-h) An \DNZZ{} example created by another experts:
    e) The video first shows the Tactical level data that reveals the player in red strokes the ball to an empty area that his opponent cannot cover.
    f) Then the video rollbacks to the previous turn and replays again.
    g) In this time, the video highlights that the player in red first uses his left hand.
    h) However, in the next movement, he switches to use his right hand to stroke the ball, and thus successfully hits the ball to the empty area.
  }
 \label{fig:case}
\end{figure*}

==> tex/_deprecated/45-visualization.tex <==
\subsection{Visualizing the Data through Recommendation}
% Based on the data level, narrative order, and data selected by the user,
\system{} integrates a visualization recommendation
engine to map the data to visuals based on the user selected narrative order (G3).
% different visual effects
% and plan the appearance orders of the augmentations (G3).

\para{Visuals---Maximum Conditional Probability.}
% Given the data selected by the user, the system should suggest proper visuals.
% There are many techniques 
% for mapping data to visuals,
Previous research proposed several methods to suggest visuals based on the data,
such as rule-based~\cite{voyager}, constraint-based~\cite{draco}, decision tree~\cite{WangSZCXMZ20}, and neural network~\cite{viznet}.
Considering our specific domain, 
we intend to use the collected videos as a prior knowledge to recommend the visuals.
Specifically, 
we model the visual mappings using conditional probability distribution: $p = f((d, v) \mid O)$,
where $d$, $v$, and $O$ is the data, visual, and narrative order, respectively.
Intuitively, this model represents the probability distribution of data-visual mappings under different narrative orders. 
This probability distribution can be estimated based on the occurrence frequency of the combinations of data, visual, and narrative orders in our corpus.
Consequently, given $d$ and $O$, 
our system will search the $v$ that maximizes $p$ and suggest it to the user.
We also use a rule-based method~\cite{voyager} as the default 
to select effective visual channels for the data
if there are no mapping records of the data under a narrative order.
Our method is simple but effective 
since it is built on the videos 
% collected 
from reputable sources,
and can be extended and optimized 
in future.

Finally, given the position of the objects in each frame are detected,
we can easily render the visual effects of the objects in the screen space.

\para{Narrative Order---Double-tracks Rendering.}
The next task is 
% After obtaining the data insights (\autoref{fig:pipeline}c),
% the system needs 
to decide the appearance order of the data in relation to the raw video.
In \system{}, we model the appearance order of different data
by using a Directed Acyclic Graph (DAG).
The DAG is constructed based on the \DN{} selected by the user.
For example, 
in \autoref{fig:pipeline}c,
if the user selects a \DNFF{},
our system will automatically add a virtual link between node $E3$ and $E4$ (\cmo{the dashed link in \autoref{fig:pipeline}d}).
% In the actual execution of the animation,
Then when executing the animation,
our system will perform a topological sort to ensure
all the prepended nodes of $E3$ are presented before animating to $E4$.
Besides, $E4$ will be flagged to avoid repeated visualizations.
Current system only implements the common patterns mentioned in Sec.~\ref{ssec:common}.

Obviously, not in all cases, a virtual link should be added between two nodes.
The addition of links between two nodes depends on their data attributes to show.
% For example, \cmo{what example?}
In our implementation, 
we use the annotations of our video corpus as prior knowledge
to decide whether a link should be added or not.
Specifically, 
before adding virtual links between two nodes 
(\emph{e.g.}, use \DNFF{} to show a player's position in $E4$ 
after showing the placement of a ball in $E3$),
we will search the corpus to ensure such pattern exists; 
otherwise, the link will not be added.
% In current version, we only implemented the common patterns mentioned in Sec.~\ref{ssec:common}.

==> tex/_deprecated/6-userstudy.tex <==

\section{User Study}

We conducted a user study to assess the usability and utility of \system{}. 
The study aimed to evaluate whether sports experts, the target users,
can create augmented table tennis videos with our system
and observe their creation process to reflect on future improvements.

\para{Participants:}
We recruited 7 table tennis experts (E1-E7; 3 male; age: 20-30, one didn't disclose)
from a university sports science department.
All experts were majored in Sports Training 
% and were professional table tennis athletes
with at least 10 years professional experiences in table tennis.
All the experts had experiences of using lightweight video editors, \emph{e.g.}, VUE~\cite{vue} but no experiences on advanced video editing tools, \emph{e.g.}, Adobe Premiere, Adobe After Effects, and Camtasia.
The scale of expert participants is consistent with similar sports visualization research~\cite{wu2017ittvis, stein2018}.
Each participant received a gift card worth \$14 at the beginning of the session, independent of their performance. 

\para{Task and Materials:}
The task required the participants to augment two table tennis videos 
with data insights they discovered.
We prepared two table tennis videos, namely, 
,
since they were selected as top 10 rallies in 2019 by ITTF~\cite{mavsboll, linvsOvt}.
A digital sheet of the design space and statistics of our corpus 
and another sheet of all the data extracted from the two videos were provided.
We also provided the participants with sketching materials,
including blank papers, printed frames of the videos, color markers, and pens.


\begin{figure}[h]
  \centering
  \includegraphics[width=0.48\textwidth]{figs/6_studyprocedure.pdf}
  \caption{The overview of the study procedure.}
 \label{fig:study_procedure}
\end{figure}

\para{Procedure:} 
The procedure is summarized in \autoref{fig:study_procedure}.
The study began with the introduction (20min) of 
the study purpose,
the concept and examples of augmented sports videos,
and the design space with 15 curated example videos.
We also played an official tutorial video of Vizrt Libero~\cite{vizrttutorial},
a state-of-the-art commercial tool,
to introduce the typical creation process of augmented sports videos.
We moved to the sketching phase (20min) when the experts had no more questions of the introduction.
The sketching phase aimed to contextualize the task
and helped the experts familiar with the raw video.
We provided the experts with all the prepared materials
and asked them to describe their interpretations of the game
and sketch the augmentations on the videos.
The experts were encouraged to augment the videos for different target users,
including proficient players, expert designers, and sports enthusiasts,
and instructed to assume that all the data was available. 
Questions and discussions were encouraged throughout the whole process.

When the experts were confirmed finishing their sketching,
we moved to the next phase and introduced \system{} (15min) with a step-by-step example.
Experts were then encouraged to explore the system (30min) and create augmentations.
For each raw video, we asked the experts to submit one augmented result. 
The study was concluded by a semi-structured interview with a 7-point Likert scale
questionnaire (15min). 
Each session was run in the lab, using a 24-inch monitor, 
with a think-aloud protocol, and lasted approximately 1.5 hours.


\subsection{Results}

\begin{figure}[h]
  \centering
  \includegraphics[width=0.49\textwidth]{figs/62_usability_chart.pdf}
  \caption{
    Experts' feedback on the usability, showing means and 95\%CIs. 
    Distributions are shown on the left.
  }
 \label{fig:author_rating}
\end{figure}

\para{Efficiency}:

\para{Effectiveness}:

\para{Satisfaction}:

\para{Usability}: Overall, our system was rated as \emph{easy to learn} ($\mu = 6.00, 95\% CI = [5.04, 6.96]$)
and \emph{easy to use} ($\mu = 6.86, 95\% CI = [6.58, 7.14] $) by the experts (\autoref{fig:author_rating}).
As commented by E3, \emph{``the system doesn't have too much complex UI''} and
\emph{``I can quickly generate augmentations by clicking several buttons.''}
Although we had never mentioned the concept of templates,
E4 pointed out that \emph{``easy, your system applies templates to the video...''}.
When we asked which part is the most difficult to learn, 
four of the experts thought was to \emph{``select proper visual effects''},
two (E4 and E5) said the concept of narrative order,
and one (E1) believed nothing was too difficult.

\para{Usefulness}:
The data-driven features---data insights and visuals recommendations---of our
system were particularly lauded by the experts 
and confirmed to be 
useful ($\mu = 6.57, 95\% CI = [5.99, 7.15]$ and $\mu = 6.71, 95\% CI = [6.35, 7.08]$, respectively).
All experts thought that the data recommendation based on narrative purposes 
was useful, which, commented by E2, was \emph{``just like a meal set''}.
E3 detailed that \emph{``it saves your time from selecting data to be presented.''}
% and the recommended data insights were meaningful,
% especially for the last three turns (reflected by five experts). 
% ``The highlighted actions in the last three turns are very reasonable. But the first three turns are less...'' (E4) We explained this was mainly due to the data extraction models we used and can be improved once more data was available.
The experts found the visualization recommendation was particularly useful
as they didn't want to \emph{``get into the details of visual mappings''}.
Besides, E4 responded that \emph{``the recommendation will be better if it can show me the comparison of different narrative orders.''}

\textbf{Satisfaction}:
The rating also reflected a high user satisfaction for the data ($\mu = 6.71, 95\% CI = [6.35, 7.08]$)
and visualization recommendations ($\mu = 6.14, 95\% CI = [5.48, 6.81]$).
The experts said the visualization recommendation \emph{``really helps guys like us (sports experts)...''}
Comments also implied further improvements of the data insights recommendation: 
\emph{``The highlighted actions in the last three turns are very reasonable. But the first three turns are less...''} (E2, E3).
We explained that this was mainly due to the data extraction models, 
which can be improved once more data was available.

% \begin{figure}[htb]
%   \centering
%   \includegraphics[width=0.49\textwidth]{figs/61_sketching.jpg}
%   \caption{
%     a) A photo of an expert in the sketching phase.
%     b) Annotations added by an expert on the printed frames of a video.
%     c) A comic strip drawn by an expert, explaining why a player wins the game.
%   }
%  \label{fig:sketching}
% \end{figure}

\para{Created Examples.}
%% sketching examples
During the sketching phase, we observed that most of the experts
were only able to draw simple lines (\autoref{fig:sketching}b) to express their ideas.
Some experts were even reluctant to sketch on the paper, except E4,
who used a comic strip (\autoref{fig:sketching}c) to introduce his idea.
%% system examples
In the system exploration phase,
the experts generated 53 augmented clips in total based on the server logs.
These clips covered all the data levels and narrative orders supported by our system, implying that the experts
had fully explored the system.
As for the 14 final submitted clips,
most of them focused (11) on the tactical data of the last 2 or 3 turns of the games
% Most of the augmentations (38) focused on the last two to three turns of the games
since ``\emph{usually the last three turns are the most important}'' (E1-7).
\autoref{fig:case} presents two examples from the experts.

\begin{figure*}[htb]
  \centering
  \includegraphics[width=\textwidth]{figs/62_case.jpg}
  \caption{
    a)-d) An \DNFF{} augmented video example created by an expert:
    a) The augmentation shows that when the player in black plans to move to the right,
    his opponent attempts to stroke the ball to the left.
    b) The player in black tries his best to return the ball.
    c) After he return the ball, his opponent strokes the ball to the right, d) which is too far away for him to return the ball. Thus, he loses this rally.
    e)-h) An \DNZZ{} example created by another experts:
    e) The video first shows the Tactical level data that reveals the player in red strokes the ball to an empty area that his opponent cannot cover.
    f) Then the video rollbacks to the previous turn and replays again.
    g) In this time, the video highlights that the player in red first uses his left hand.
    h) However, in the next movement, he switches to use his right hand to stroke the ball, and thus successfully hits the ball to the empty area.
  }
 \label{fig:case}
\end{figure*}

% \begin{figure}[h]
%   \centering
%   \includegraphics[width=0.49\textwidth]{figs/62_audience.pdf}
%   \caption{ Overall ratings of the two random selected augmented videos created by the experts, indicating the positive feedback from 23 sports fans.
%   }
%  \label{fig:audience_rating}
% \end{figure}

% \textbf{Audiences feedback.}
% We further conducted an online survey to qualitatively
% assessed the augmented clips created by the experts from the audience's angle.
% Given some augmented clips have the similar content,
% we first deduplicated them
% and then randomly selected one clip for each video.
% The two clips, together with their original version and a post-watch survey (drawn from~\cite{WangSZCXMZ20}),
% were posted to a digital forum of a university.
% We only invited table tennis fans 
% who we considered as the target users of the augmented videos.
% \autoref{fig:audience_rating} shows the results collected from 23 participants with a very diverse background (13 majors).
% Overall, the participants provided positive feedback with respect 
% to both the visual effects data content.
% Given the augmented videos were created by our proof-of-concept system without further polishing, 
% we consider these feedbacks to indicate the promising of our system.


\subsection{Observations and Feedback.}
Now we reflect on the interesting observations and feedback, 
which we believe imply future opportunities.

\textbf{Design Space for atypical designers.}
We consider the sports expert in our scenario is a kind of typical designers:
on the one hand, the sports experts are not novices, and the content of the augmented videos is usually decided by them; 
on the other hand, the sports experts are not designers, and lack sufficient skills and knowledge
to create a video.
Thus, we are interested in the sports experts' feedback on the design space.
In the interview,
all experts confirmed the usefulness of the design space, especially the \DD{}.
\emph{``This helps us know our audience...,''} commented by E4, who used to explain table tennis matches with too many tactical details to his friends.
As for the \DN{}, some experts thought that it was \emph{``too fancy''}
and believed only using \emph{linear} and \emph{flashforward} were enough.
But they also added that \emph{``maybe audiences will like it...''}
These responses were consistent with our expectations that the sports experts focus more on the
data aspect instead of the visual one.
We considered this feedback also indicates that 
the design of authoring systems for sports experts 
should provide more automation for the visual part than the data part.


%% demands
\textbf{Data analysis---Translate high level findings into specific data.}
One unique characteristic of augmented sports videos is that
a sports video is both the source of data
and the canvas for showing the data,
which makes the data analysis and communication inseparable in creating augmented sports videos.
We did observe that experts paused and analyzed the key period of the videos, 
took notes of the players and ball,
and then augmented the video based on their notes.
However, we noticed that the experts' analytic findings 
were usually very abstract
and even difficult to find data equivalent, \emph{e.g.}, \emph{``I can see something in his eyes, he is going to lose''} (E5) and \emph{``his pace is messed up''} (E2)
Given the highly abstract nature of these findings,
the experts usually needed to translate them into specific data
and then further visualize them; or sometimes they just gave up.
In such a case, 
our data insights recommendation features can inspire the experts
and helps them discover other interesting patterns.
A promising future direction is to explore the way to \textbf{translate
the experts' high level findings into specific data}.
To achieve this, a possible solution is to utilize
natural language processing techniques, which have already been employed in some creativity support tools~\cite{DBLP:conf/chi/KimDAH19, DBLP:conf/chi/LaputDWCALA13}.

% Thus, the experts usually needed to figured out a proper way to present 
% these findings in the videos or just gave up.
% Prior research has proposed to bridge the gap between analysis and communication~\cite{chen2020, kim2020} 
% by visually storing the analytic findings from visual analytics systems.
% We consider the bottleneck is that the findings from a video can be very abstract
% while the presentations in a video are usually very concrete.
% How to close this gap requires future research.

%% direct manipulation + speech
\textbf{Data visualization---Select the data, instead of visualizations.}
Sports experts are more familiar with data instead of visualizations.
In the study, we observed that the experts tended to design the augmented videos from a data perspective and considered less on the visuals.
For example, the experts frequently said that \emph{``show the ball trajectory/ball placements/player position''}. 
However, when we asked them \emph{``by using what?''},
most of them responded that \emph{``just use the positions''}, \emph{``not important''} or \emph{``I don't know.''}
In the interview, 
we proposed two system designs that allow the experts to
1) \emph{``select a graphical mark to annotate a player's position''}
or 2) \emph{``select a player's position attribute and highlight it with system suggested marks''}.
All the experts preferred the last one. 
This also reflected the usefulness of our visualizations recommendation for the experts.
However, most commercial tools adopt the first method,
which ask the user to \textbf{select a mark} to annotate the data 
rather than \textbf{select a data} to be highlighted.
Object-oriented UI design~\cite{dataink, marvist},
which allows the experts to create visual mappings through direct manipulations,
can be a potential solution to address this issue.

% Our systemalso involves certain inherent limitations.   First,  the VR headset isbulky and thus increases the physical workload. The experts generallyneeded to take a break every 15 minutes during the studies.  Second,the VR environment separates the user from the real world, causinghesitation from the user to walk around before getting used to theenvironment.  We observed that at the beginning of the studies, theexperts carefully attempted to move their feet to avoid falling to thefloor.  They became confident to move in the simulated court whenthey got used to the immersive environment. After a discussion withthe experts, we proposed to use some reference points to relate thevirtuality and reality. For example, we can put a chair in the real roomand use a similar virtual chair in the virtual court to indicate the positionof the user in relation to the real room. Third, the controllers cannotsimulate the haptic feedback of stroking a shuttle, thus requiring theexperts to spend a certain time to adapt.

==> tex/_deprecated/6-userstudy2.tex <==
\section{User Study}

We conducted a user study to assess the usability of \system{}. 
The study aimed to evaluate whether sports analysts, the target users,
can create augmented table tennis videos with our system
and observe their creation process to reflect on future improvements.
We did not run a comparative study with, \emph{e.g.}, Adobe Premiere, as a baseline
since the features of our system do not exist in Premiere or clearly faster.

\para{Participants}:
We recruited 7 table tennis analysts (E1-E7; \cmo{3 male; age: 20-30}, one didn't disclose)
from a university sports science department.
All experts were majored in Sports Training 
with proficient experience in analyzing table tennis matches.
All the experts had experiences of using lightweight video editors, \emph{e.g.}, VUE~\cite{vue} but no experiences on advanced video editing tools, \emph{e.g.}, Adobe Premiere and Camtasia.
The scale of expert participants is consistent with similar sports visualization research~\cite{wu2017ittvis, stein2018}.
Each participant received a gift card worth \$14 at the beginning of the session, independent of their performance. 

\para{Tasks}:
The participants were asked to reproduce two augmented videos by using our system.
We prepared two augmented videos
based on two ITTF top 10 rallies in 2019~\cite{}:
\textbf{T1} (\autoref{fig:case}b) is augmented by event-level data and presented by FlashForaward;
and \textbf{T2} (\autoref{fig:case}c) is augmented by tactic-level data and presented by TimeFork.
% table tennis videos (\emph{i.e.}, \cmo{xxx})
% which were selected as top 10 rallies in 2019 by ITTF~\cite{mavsboll, linvsOvt}.
% The resulted augment videos cover two data levels (\emph{i.e.} object- and tactic-levels) 
% and three most frequently used narrative orders (\emph{i.e.}, Linear, FlashForward, and TimeFork).
For each video,
we provided the resulted augmented video,
background information,
a manual of the system,
a digital instruction of the design space,
and the data extracted from the video.
For the training task, 
we further prepared another augmented video (\autoref{fig:case}\cmo{a}), \textbf{T0},
which is also created based on a ITTF top 10 rallies and covers all the features in \textbf{T1} and \textbf{T2}.

% \begin{figure}[h]
%   \centering
%   \includegraphics[width=0.48\textwidth]{figs/6_studyprocedure.png}
%   \caption{The overview of the study procedure.}
%  \label{fig:study_procedure}
% \end{figure}

\para{Procedure}: 
The procedure is summarized in \autoref{fig:study_procedure}.
The study began with the introduction (15min) of 
the study purpose,
the concept and examples of augmented sports videos,
and the design space with 15 curated example videos.
We also played an official tutorial video of Vizrt Libero~\cite{vizrttutorial},
a state-of-the-art commercial tool,
to introduce the typical creation process of augmented sports videos.
We moved to the training phase (20min) when the experts had no more questions of the introduction.
The participants were walked through with a step-by-step instruction to reproduce \textbf{T0} (\autoref{fig:case}\cmo{a}).
Questions and discussions were encouraged throughout the whole process.
% We moved to the sketching phase (20min) when the experts had no more questions of the introduction.
% The sketching phase aimed to contextualize the task
% and helped the experts familiar with the raw video.
% We provided the experts with all the prepared materials
% and asked them to describe their interpretations of the game
% and sketch the augmentations on the videos.
% The experts were encouraged to augment the videos for different target users,
% including proficient players, expert designers, and sports enthusiasts,
% and instructed to assume that all the data was available. 

After the training, participants were 
provided with the materials of the two reproduction tasks, \textbf{T1} and \textbf{T2} (15min for each).
We encouraged them to ask questions about and get familiar with the materials.
A task was started when a participant was confident and confirmed to begin, 
and ended when the participant confirmed finishing. 
To assess the efficiency and effectiveness of the system,
we recorded the completion \emph{time} and \emph{correctness} for each task.
A task is failed if the participant cannot reproduce the video in 15 minutes.
A successful reproduction should correctly reproduce the 
the data level, narrative order, and all the visual-data mappings of the given video.
All measures were explicitly explained before the tasks.

The session ended with a semi-structured interview and a post-study questionnaire (15min).
Each session was run in the lab, using a 24-inch monitor, 
with a think-aloud protocol, and lasted around 90 minutes.
% 7-point Likert scale
% The correct points of \textbf{T1} and \textbf{T2} are 7 and 11, respectively,
% including 


\subsection{Results}
All participants could successfully reproduce the two augmented videos \cmo{in a few minutes}
(\textbf{T1}: $\mu = 6.00, 95\%$ $CI = [5.04, 6.96]$; 
\textbf{T2}: $\mu = 6.00, 95\%$ $CI = [5.04, 6.96]$).
We did observe that some participants (P1, P3, P4) could not correctly reproduce
the videos in the first place. 
But they could interatively refine the results by checking with the expected output
and finally create the correct ones.
This is also the reason why these participants took longer time to finish the tasks.
Besides, we also noticed that P2 and P5 explored other augmentation during the tasks
even they had already successfully created the results, leading to extra time to finish the tasks.
Overall, these quantitative results demonstrate the effectiveness and efficiency of our system.
We also collected and summarized the participants' qualitative feedback:

\begin{figure}[h]
  \centering
  \includegraphics[width=0.49\textwidth]{figs/62_usability_chart.png}
  \caption{
    Experts' feedback on the usability, showing means and 95\% CIs. 
    Distributions are shown on the left.
  }
 \label{fig:author_rating}
\end{figure}

\para{Usability}: Overall, our system was rated as \emph{easy to learn} ($\mu = 6.00, 95\% CI = [5.14, 6.86]$)
and \emph{easy to use} ($\mu = 6.86, 95\% CI = [6.58, 7.14] $) by the participants (\autoref{fig:author_rating}).
The participants (P1-4, P6) commented that \emph{``Compared to mainstream video editors, this system allows me to do more with less efforts.''} P3 provided in detail that \emph{``I have used other video editors...I can\'t imagine how can I use them to create augmented videos...''}
When we asked the participants whether they need more customization of the augmentations 
(\emph{e.g.}, the order of visual effects in flashforward),
most of them agreed that on one hand, the tool should 
strike a balance between customizability and simplicity
as their goal is to \emph{``rapid prototyping.''};
on the other hand, the tool should allow editing of the details when the user needs to.
% allow controlling the details
% which part is the most difficult to learn,
% four of the participants thought was to \emph{``''}
% two (P3 and P7) 
% As commented by P3, \emph{``the system doesn't have too much complex UI''} and
% \emph{``I can quickly generate augmentations by clicking several buttons.''}
% Although we had never mentioned the concept of templates,
% P4 pointed out that \emph{``your system applies templates to the video...''}.
% When we asked which part is the most difficult to learn, 
% four of the experts thought was to \emph{``select proper visual effects''},
% two (E4 and E5) said the concept of narrative order,
% and one (E1) believed nothing was too difficult.

\para{Usefulness}:
The key designs---data extractor, direct manipulation user interface, and visuals recommendation--of our
% The data-driven features---data insights and visuals recommendations---of our
system were particularly lauded by the experts 
and confirmed to be 
useful ($\mu = 6.29, 95\%$ $CI = [5.73, 6.85]$, $\mu = 6.86, 95\%$ $CI = [6.58, 7.14]$, and $\mu = 6.57, 95\%$ $CI = [6.00, 7.15]$, respectively).
The participants thought that extracting and organizing data based on data levels were useful.
P2 commented that \emph{``organizing data into the three levels is not surprised to me, but connecting them to different narrative purposes inspires me a lot.''}
All the participants spoke highly of how we support the augmentation through direct manipulation.
\emph{``Clearly revealing the object to be augmented''} is the main reason why the participants favored it.
P7 further pointed out that the design makes the task \emph{``cognitively easy.''}
The experts found the visualization recommendation was particularly useful
as they \emph{``did not familiar with mapping data to visuals.''}
% \emph{``Although I can do that by trial and error, it is time consuming.''}
Besides, P5 suggested to allow \emph{``comparison between different recommendations.''}

\para{Satisfaction}:
The rating also reflected a high user satisfaction for the data extractor ($\mu = 6.29, 95\% CI = [5.36, 7.20]$),
direct manipulation design ($\mu = 6.43, 95\% CI = [5.85, 7.00]$),
and visualization recommendation ($\mu = 6.43, 95\% CI = [5.85, 7.00]$).
The participants said that the direct manipulation design was \emph{``intuitive''} (P1-P7)
and the visualization recommendation \emph{``helps guys like us (sports analysts)...''} (P1, P6)
Comments also implied further improvements of the data extractor:
\emph{``The available tactic data is a bit limited..''} (P3, P6)
We explained that this was mainly due to the limitations of ML models
and our system allows the user to import external tactic data.


\subsection{Observations and Feedback}
We reflect on the observations of the study and interview feedback,
which imply future opportunities.

\para{The advantages of presenting analytical insights through augmented videos.}
We were interested in how the participants usually presented their analytical insights of a match
and what are the advantages of using augmented videos.
All the participants responded that voiceover on the video is the most common way to present their findings.
They also prepared slides to add graphical annotations and text descriptions to the video.
Some participants (P3, P5, P6) mentioned that they would created simple charts, such as bar and pie chart, to visualize the data.
Compared to these methods, the main benefit of augmented videos is \emph{``intuitive.''} (P1-P7)
Specifically, the augmented videos can 
reduce the cognitive load of the audience to understand and connect the complex data to the physical context.
P2 explained that \emph{``the audiences do not need to imagine and can directly see what I am talking in the video.''}
Another advantage is \emph{``(the augmented video) can increase the memorability.''} (P1, P3-P7),
which is particularly useful for the players,
since \emph{``the player usually can only recall the visual scenes rather than the numbers in a match.''} (P5) 

\para{The necessity of bridging the gap between analyzing and communicating data.}
While visual analytics systems have been increasingly used for data analysis,
it remains challenging for the analysts to create visual designs to communicate their analytical findings.
For example, although all the participants expressed their favor of augmented videos, % to present analytical findings,
they had never created augmented videos before 
since \emph{``it is too complicated to create them by using video editors.''} (P2)
P7 detailed that \emph{``the design tools mainly focus on the visual parts''} 
so that the analyst have to \emph{``manually map the data insights to the visual elements.''}
Thus, all the participants appreciated that our system allows data-driven other than graphics-driven design
as \emph{``the ultimate goal of drawing a curve on the video is to present the trajectory data.''} (P7)
Nonetheless, the participants also suggested that our system should be integrated more closely
with visual analytics systems, \emph{e.g.}, instead of asking the analyst to manually configure the visual mappings,
the system should allow the analyst to import the analytical findings
and automatically generate augment videos.
We consider this suggestion as 
an important future direction of bridging the gap between visual analytics and storytelling.

\para{Translating high-level insights into specific data.}
During the reproduction tasks, we observed a main obstacle for the participants
is to translate a high-level insight presented by the targeted video into specific data.
For example, the participants perceived that \autoref{fig:case}c1 is showing a tactic of \emph{attacking on both sides}.
However, to reproduce this clip,
the participants needed to break down this tactic into specific data 
such as \emph{ball trajectory}, \emph{moving direction} of the ball and player.
This ``translation'' process usually led to a trial-and-error situation.
In the interview, 
the participants commented that this process is similar to a reverse analysis 
in which the analyst needs to \emph{``generate data from insights.''} (P7)
Moreover, P1 provided that in some cases there is no data equivalent of an insights, \emph{e.g.}, \emph{``the player is in low spirits.''}
This finding implies future study to translate the analyst's high-level findings into specific data,
which is also an important component to bridge the gap between visual analytics and storytelling.
A potential solution is to leverage natural language processing techniques, 
which have already been employed in some creativity support tools~\cite{DBLP:conf/chi/KimDAH19, DBLP:conf/chi/LaputDWCALA13}.

\para{Suggestions.}
The participants also identified some limitations of \system{} and suggested improvements.
Most limitations were related to system engineering maturity,
% as our system is not meant to be a fully functional video editor.
\emph{e.g.},
transition animations between clips were not supported;
some parameters (\emph{e.g.}, playback rate) were fixed to default values.
Our system also involves certain inherent limitations due to the underlying ML models.
First, the input video needs to cover the whole court with a fixed camera angle.
Although this is the common case for racket sports,
the videos of other team sports such as football and basketball do not satisfy this requirement,
which requires additional steps to concatenate and map different views into a panoramic view~\cite{stein2017bring}.
Second, the data extracted from the video is still limited,
\emph{e.g.}, the server type, hitting area, and other historical data are unavailable.
To mitigate this issue, 
we allow the analyst to import data from dedicated data annotation systems (\emph{e.g.}, \cmo{})
in which the data is also organized into three data levels.
Third, the system only supports augmentation in the screen space instead of the world space.
In other words, our system did not reconstruct the 3D scene of the video 
and thus cannot properly handle the z-order and occlusions of elements.


% Some limitations indicate promising improvements.
% For example, the experts suggested that not only the data levels but also the visual effects should also be recommended based on narrative purposes, as \emph{``athletes don't need such fancy visualizations.''} (E2)

% However, we noticed that the experts' analytic findings were usually very abstract
% and even difficult to find data equivalent, \emph{e.g.}, \emph{``I can see something in his eyes, he is going to lose''} (E5) and \emph{``his pace is messed up''} (E2)
% Given the highly abstract nature of these findings,
% the experts usually needed to translate them into specific data
% and then further visualize them; or sometimes they just gave up.

% In such a case, 
% our data insights recommendation features can inspire the experts
% and helps them discover other interesting patterns.

% A promising future direction is to explore the way to \textbf{translate
% the experts' high level findings into specific data}.

% One unique characteristic of augmented sports videos is that
% a sports video is both the source of data
% and the canvas for showing the data,
% which makes the data analysis and communication inseparable in creating augmented sports videos.
% We did observe that experts paused and analyzed the key period of the videos, 
% took notes of the players and ball,
% and then augmented the video based on their notes.


% This implies that the authoring tools for communicating data
% should focus on data-driven other than graphics-driven design.

% To communicate the analytical findings, visual storytelling is considered as an effective and engaging method.
% creating effective visual storytelling is a demanding task for the domain experts, 
% who usually lack sufficient design expertise.
% For example, 
% the authoring tools (\emph{e.g.}, graphic design tools, video editor)
% are complex and have a steep learning curve.
% it remains challenging for the experts to present the findings as the analytical visualizations may be too complex.
% On the other hand,  to communicate analytical insights.
% Thus, helping domain experts to present their analytical insights is in great demand.
% Potential solution can be twofold:
% either adding storytelling features to visual analytics systems~\cite{}
% or adding data-driven supports to graphic or video design tools~\cite{}.
% developing dedicated storytelling authoring tools tailored to domain experts.

% Many visual analytics systems have been developed to support analysts to explore and make sense with data in various domain.
% We consider the sports expert in our scenario is a kind of typical designers:
% on the one hand, the sports experts are not novices, and the content of the augmented videos is usually decided by them; 
% on the other hand, the sports experts are not designers, and lack sufficient skills and knowledge
% to create a video.
% Thus, we are interested in the sports experts' feedback on the design space.
% In the interview,
% all experts confirmed the usefulness of the design space, especially the \DD{}.
% \emph{``This helps us know our audience...,''} commented by E4, who used to explain table tennis matches with too many tactical details to his friends.
% As for the \DN{}, some experts thought that it was \emph{``too fancy''}
% and believed only using \emph{linear} and \emph{flashforward} were enough.
% But they also added that \emph{``maybe audiences will like it...''}
% These responses were consistent with our expectations that the sports experts focus more on the
% data aspect instead of the visual one.
% We considered this feedback also indicates that 
% the design of authoring systems for sports experts 
% should provide more automation for the visual part than the data part.

% Many visual storytelling authoring tools (\emph{e.g.}, DataShot~\cite{}, \cmo{XXX}~\cite{})
% feature automated data stories recommendation to help the user discover interesting data patterns.
% In the prior version, \system{} also integrated a data insights recommendation system.
% The recommendation engine is adapted from DataShot and recommended data insights (\emph{e.g.}, extreme, rank, trend, association) based on statistical significance.

%% show to the participants

%% feedback from the participants

%% how to create effective data insight recommendation


%% demands
% \para{Data visualization---Select the data, instead of visualizations.}
% Sports experts are more familiar with data instead of visualizations.
% In the study, we observed that the experts tended to design the augmented videos from a data perspective and considered less on the visuals.
% For example, the experts frequently said that \emph{``show the ball trajectory/ball placements/player position''}. 
% However, when we asked them \emph{``by using what?''},
% most of them responded that \emph{``just use the positions''}, \emph{``not important''} or \emph{``I don't know.''}
% In the interview, 
% we proposed two system designs that allow the experts to
% 1) \emph{``select a graphical mark to annotate a player's position''}
% or 2) \emph{``select a player's position attribute and highlight it with system suggested marks''}.
% All the experts preferred the last one. 
% This also reflected the usefulness of our visualizations recommendation for the experts.
% However, most commercial tools adopt the first method,
% which ask the user to \textbf{select a mark} to annotate the data 
% rather than \textbf{select a data} to be highlighted.
% Object-oriented UI design~\cite{dataink, marvist},
% which allows the experts to create visual mappings through direct manipulations,
% can be a potential solution to address this issue.

% Thus, the experts usually needed to figured out a proper way to present 
% these findings in the videos or just gave up.
% Prior research has proposed to bridge the gap between analysis and communication~\cite{chen2020, kim2020} 
% by visually storing the analytic findings from visual analytics systems.
% We consider the bottleneck is that the findings from a video can be very abstract
% while the presentations in a video are usually very concrete.
% How to close this gap requires future research.

% Our systemalso involves certain inherent limitations.   First,  the VR headset isbulky and thus increases the physical workload. The experts generallyneeded to take a break every 15 minutes during the studies.  Second,the VR environment separates the user from the real world, causinghesitation from the user to walk around before getting used to theenvironment.  We observed that at the beginning of the studies, theexperts carefully attempted to move their feet to avoid falling to thefloor.  They became confident to move in the simulated court whenthey got used to the immersive environment. After a discussion withthe experts, we proposed to use some reference points to relate thevirtuality and reality. For example, we can put a chair in the real roomand use a similar virtual chair in the virtual court to indicate the positionof the user in relation to the real room. Third, the controllers cannotsimulate the haptic feedback of stroking a shuttle, thus requiring theexperts to spend a certain time to adapt.

==> tex/_deprecated/_deprecated.tex <==

\section{Using the Style Template}

\begin{itemize}
\item If you receive compilation errors along the lines of ``\texttt{Package ifpdf Error: Name clash, \textbackslash ifpdf is already defined}'' then please add a new line ``\texttt{\textbackslash let\textbackslash ifpdf\textbackslash relax}'' right after the ``\texttt{\textbackslash documentclass[journal]\{vgtc\}}'' call. Note that your error is due to packages you use that define ``\texttt{\textbackslash ifpdf}'' which is obsolete (the result is that \texttt{\textbackslash ifpdf} is defined twice); these packages should be changed to use ifpdf package instead.
\item Note that each author's affiliations have to be provided in the author footer on the bottom-left corner of the first page. It is permitted to merge two or more people from the same institution as long as they are shown in the same order as in the overall author sequence on the top of the first page. For example, if authors A, B, C, and D are from institutions 1, 2, 1, and 2, respectively, then it is ok to use 2 bullets as follows:
\begin{itemize}
\item A and C are with Institution 1. E-mail: \{a\,$|$\,c\}@i1.com\,.
\item B and D are with Institution 2. E-mail: \{b\,$|$\,d\}@i2.org\,.
\end{itemize}
\item The style uses the hyperref package, thus turns references into internal links. We thus recommend to make use of the ``\texttt{\textbackslash autoref\{reference\}}'' call (instead of ``\texttt{Figure\~{}\textbackslash ref\{reference\}}'' or similar) since ``\texttt{\textbackslash autoref\{reference\}}'' turns the entire reference into an internal link, not just the number. Examples: \autoref{fig:sample} and \autoref{tab:vis_papers}.
\item The style automatically looks for image files with the correct extension (eps for regular \LaTeX; pdf, png, and jpg for pdf\LaTeX), in a set of given subfolders (figures/, pictures/, images/). It is thus sufficient to use ``\texttt{\textbackslash includegraphics\{CypressView\}}'' (instead of ``\texttt{\textbackslash includegraphics\{pictures/CypressView.jpg\}}'').
\item For adding hyperlinks and DOIs to the list of references, you can use ``\texttt{\textbackslash bibliographystyle\{abbrv-doi-hyperref-narrow\}}'' (instead of ``\texttt{\textbackslash bibliographystyle\{abbrv\}}''). It uses the doi and url fields in a bib\TeX\ entry and turns the entire reference into a link, giving priority to the doi. The doi can be entered with or without the ``\texttt{http://dx.doi.org/}'' url part. See the examples in the bib\TeX\ file and the bibliography at the end of this template.\\[1em]
\textbf{Note 1:} occasionally (for some \LaTeX\ distributions) this hyper-linked bib\TeX\ style may lead to \textbf{compilation errors} (``\texttt{pdfendlink ended up in different nesting level ...}'') if a reference entry is broken across two pages (due to a bug in hyperref). In this case make sure you have the latest version of the hyperref package (i.\,e., update your \LaTeX\ installation/packages) or, alternatively, revert back to ``\texttt{\textbackslash bibliographystyle\{abbrv-doi-narrow\}}'' (at the expense of removing hyperlinks from the bibliography) and try ``\texttt{\textbackslash bibliographystyle\{abbrv-doi-hyperref-narrow\}}'' again after some more editing.\\[1em]
\textbf{Note 2:} the ``\texttt{-narrow}'' versions of the bibliography style use the font ``PTSansNarrow-TLF'' for typesetting the DOIs in a compact way. This font needs to be available on your \LaTeX\ system. It is part of the \href{https://www.ctan.org/pkg/paratype}{``paratype'' package}, and many distributions (such as MikTeX) have it automatically installed. If you do not have this package yet and want to use a ``\texttt{-narrow}'' bibliography style then use your \LaTeX\ system's package installer to add it. If this is not possible you can also revert to the respective bibliography styles without the ``\texttt{-narrow}'' in the file name.\\[1em]
DVI-based processes to compile the template apparently cannot handle the different font so, by default, the template file uses the \texttt{abbrv-doi} bibliography style but the compiled PDF shows you the effect of the \texttt{abbrv-doi-hyperref-narrow} style.
\end{itemize}


\section{Bibliography Instructions}

\begin{itemize}
\item Sort all bibliographic entries alphabetically but the last name of the first author. This \LaTeX/bib\TeX\ template takes care of this sorting automatically.
\item Merge multiple references into one; e.\,g., use \cite{Max:1995:OMF,Kitware:2003} (not \cite{Kitware:2003}\cite{Max:1995:OMF}). Within each set of multiple references, the references should be sorted in ascending order. This \LaTeX/bib\TeX\ template takes care of both the merging and the sorting automatically.
\item Verify all data obtained from digital libraries, even ACM's DL and IEEE Xplore  etc.\ are sometimes wrong or incomplete.
\item Do not trust bibliographic data from other services such as Mendeley.com, Google Scholar, or similar; these are even more likely to be incorrect or incomplete.
\item Articles in journal---items to include:
  \begin{itemize}
  \item author names
	\item title
	\item journal name
	\item year
	\item volume
	\item number
	\item month of publication as variable name (i.\,e., \{jan\} for January, etc.; month ranges using \{jan \#\{/\}\# feb\} or \{jan \#\{-{}-\}\# feb\})
  \end{itemize}
\item use journal names in proper style: correct: ``IEEE Transactions on Visualization and Computer Graphics'', incorrect: ``Visualization and Computer Graphics, IEEE Transactions on''
\item Papers in proceedings---items to include:
  \begin{itemize}
  \item author names
	\item title
	\item abbreviated proceedings name: e.\,g., ``Proc.\textbackslash{} CONF\_ACRONYNM'' without the year; example: ``Proc.\textbackslash{} CHI'', ``Proc.\textbackslash{} 3DUI'', ``Proc.\textbackslash{} Eurographics'', ``Proc.\textbackslash{} EuroVis''
	\item year
	\item publisher
	\item town with country of publisher (the town can be abbreviated for well-known towns such as New York or Berlin)
  \end{itemize}
\item article/paper title convention: refrain from using curly brackets, except for acronyms/proper names/words following dashes/question marks etc.; example:
\begin{itemize}
	\item paper ``Marching Cubes: A High Resolution 3D Surface Construction Algorithm''
	\item should be entered as ``\{M\}arching \{C\}ubes: A High Resolution \{3D\} Surface Construction Algorithm'' or  ``\{M\}arching \{C\}ubes: A high resolution \{3D\} surface construction algorithm''
	\item will be typeset as ``Marching Cubes: A high resolution 3D surface construction algorithm''
\end{itemize}
\item for all entries
\begin{itemize}
	\item DOI can be entered in the DOI field as plain DOI number or as DOI url; alternative: a url in the URL field
	\item provide full page ranges AA-{}-BB
\end{itemize}
\item when citing references, do not use the reference as a sentence object; e.\,g., wrong: ``In \cite{Lorensen:1987:MCA} the authors describe \dots'', correct: ``Lorensen and Cline \cite{Lorensen:1987:MCA} describe \dots''
\end{itemize}

\section{Example Section}

Lorem\marginpar{\small You can use the margins for comments while editing the submission, but please remove the marginpar comments for submission.} ipsum dolor sit amet, consetetur sadipscing elitr, sed diam
nonumy eirmod tempor invidunt ut labore et dolore magna aliquyam erat,
sed diam voluptua. At vero eos et accusam et justo duo dolores et ea
rebum. Stet clita kasd gubergren, no sea takimata sanctus est Lorem
ipsum dolor sit amet. Lorem ipsum dolor sit amet, consetetur
sadipscing elitr, sed diam nonumy eirmod tempor invidunt ut labore et
dolore magna aliquyam erat, sed diam
voluptua~\cite{Kitware:2003,Max:1995:OMF}. At vero eos et accusam et
justo duo dolores et ea rebum. Stet clita kasd gubergren, no sea
takimata sanctus est Lorem ipsum dolor sit amet. Lorem ipsum dolor sit
amet, consetetur sadipscing elitr, sed diam nonumy eirmod tempor
invidunt ut labore et dolore magna aliquyam erat, sed diam
voluptua. At vero eos et accusam et justo duo dolores et ea
rebum. Stet clita kasd gubergren, no sea takimata sanctus est.

\section{Exposition}

Duis autem vel eum iriure dolor in hendrerit in vulputate velit esse
molestie consequat, vel illum dolore eu feugiat nulla facilisis at
vero eros et accumsan et iusto odio dignissim qui blandit praesent
luptatum zzril delenit augue duis dolore te feugait nulla
facilisi. Lorem ipsum dolor sit amet, consectetuer adipiscing elit,
sed diam nonummy nibh euismod tincidunt ut laoreet dolore magna
aliquam erat volutpat~\cite{Kindlmann:1999:SAG}.

\begin{equation}
\sum_{j=1}^{z} j = \frac{z(z+1)}{2}
\end{equation}

Lorem ipsum dolor sit amet, consetetur sadipscing elitr, sed diam
nonumy eirmod tempor invidunt ut labore et dolore magna aliquyam erat,
sed diam voluptua. At vero eos et accusam et justo duo dolores et ea
rebum. Stet clita kasd gubergren, no sea takimata sanctus est Lorem
ipsum dolor sit amet. Lorem ipsum dolor sit amet, consetetur
sadipscing elitr, sed diam nonumy eirmod tempor invidunt ut labore et
dolore magna aliquyam erat, sed diam voluptua. At vero eos et accusam
et justo duo dolores et ea rebum. Stet clita kasd gubergren, no sea
takimata sanctus est Lorem ipsum dolor sit amet.

\subsection{Lorem ipsum}

Lorem ipsum dolor sit amet (see \autoref{tab:vis_papers}), consetetur sadipscing elitr, sed diam
nonumy eirmod tempor invidunt ut labore et dolore magna aliquyam erat,
sed diam voluptua. At vero eos et accusam et justo duo dolores et ea
rebum. Stet clita kasd gubergren, no sea takimata sanctus est Lorem
ipsum dolor sit amet. Lorem ipsum dolor sit amet, consetetur
sadipscing elitr, sed diam nonumy eirmod tempor invidunt ut labore et
dolore magna aliquyam erat, sed diam voluptua. At vero eos et accusam
et justo duo dolores et ea rebum. Stet clita kasd gubergren, no sea
takimata sanctus est Lorem ipsum dolor sit amet. Lorem ipsum dolor sit
amet, consetetur sadipscing elitr, sed diam nonumy eirmod tempor
invidunt ut labore et dolore magna aliquyam erat, sed diam
voluptua. At vero eos et accusam et justo duo dolores et ea
rebum. 

\begin{table}[tb]
  \caption{VIS/VisWeek accepted/presented papers: 1990--2016.}
  \label{tab:vis_papers}
  \scriptsize%
	\centering%
  \begin{tabu}{%
	r%
	*{7}{c}%
	*{2}{r}%
	}
  \toprule
   year & \rotatebox{90}{Vis/SciVis} &   \rotatebox{90}{SciVis conf} &   \rotatebox{90}{InfoVis} &   \rotatebox{90}{VAST} &   \rotatebox{90}{VAST conf} &   \rotatebox{90}{TVCG @ VIS} &   \rotatebox{90}{CG\&A @ VIS} &   \rotatebox{90}{VIS/VisWeek} \rotatebox{90}{incl. TVCG/CG\&A}   &   \rotatebox{90}{VIS/VisWeek} \rotatebox{90}{w/o TVCG/CG\&A}   \\
  \midrule
	2016 & 30 &   & 37 & 33 & 15 & 23 & 10 & 148 & 115 \\
  2015 & 33 & 9 & 38 & 33 & 14 & 17 & 15 & 159 & 127 \\
  2014 & 34 &   & 45 & 33 & 21 & 20 &   & 153 & 133 \\
  2013 & 31 &   & 38 & 32 &   & 20 &   & 121 & 101 \\
  2012 & 42 &   & 44 & 30 &   & 23 &   & 139 & 116 \\
  2011 & 49 &   & 44 & 26 &   & 20 &   & 139 & 119 \\
  2010 & 48 &   & 35 & 26 &   &   &   & 109 & 109 \\
  2009 & 54 &   & 37 & 26 &   &   &   & 117 & 117 \\
  2008 & 50 &   & 28 & 21 &   &   &   & 99 & 99 \\
  2007 & 56 &   & 27 & 24 &   &   &   & 107 & 107 \\
  2006 & 63 &   & 24 & 26 &   &   &   & 113 & 113 \\
  2005 & 88 &   & 31 &   &   &   &   & 119 & 119 \\
  2004 & 70 &   & 27 &   &   &   &   & 97 & 97 \\
  2003 & 74 &   & 29 &   &   &   &   & 103 & 103 \\
  2002 & 78 &   & 23 &   &   &   &   & 101 & 101 \\
  2001 & 74 &   & 22 &   &   &   &   & 96 & 96 \\
  2000 & 73 &   & 20 &   &   &   &   & 93 & 93 \\
  1999 & 69 &   & 19 &   &   &   &   & 88 & 88 \\
  1998 & 72 &   & 18 &   &   &   &   & 90 & 90 \\
  1997 & 72 &   & 16 &   &   &   &   & 88 & 88 \\
  1996 & 65 &   & 12 &   &   &   &   & 77 & 77 \\
  1995 & 56 &   & 18 &   &   &   &   & 74 & 74 \\
  1994 & 53 &   &   &   &   &   &   & 53 & 53 \\
  1993 & 55 &   &   &   &   &   &   & 55 & 55 \\
  1992 & 53 &   &   &   &   &   &   & 53 & 53 \\
  1991 & 50 &   &   &   &   &   &   & 50 & 50 \\
  1990 & 53 &   &   &   &   &   &   & 53 & 53 \\
  \midrule
  \textbf{sum} & \textbf{1545} & \textbf{9} & \textbf{632} & \textbf{310} & \textbf{50} & \textbf{123} & \textbf{25} & \textbf{2694} & \textbf{2546} \\
  \bottomrule
  \end{tabu}%
\end{table}

\subsection{Mezcal Head}

Lorem ipsum dolor sit amet (see \autoref{fig:sample}), consetetur sadipscing elitr, sed diam
nonumy eirmod tempor invidunt ut labore et dolore magna aliquyam erat,
sed diam voluptua. At vero eos et accusam et justo duo dolores et ea
rebum. Stet clita kasd gubergren, no sea takimata sanctus est Lorem
ipsum dolor sit amet. Lorem ipsum dolor sit amet, consetetur
sadipscing elitr, sed diam nonumy eirmod tempor invidunt ut labore et
dolore magna aliquyam erat, sed diam voluptua. At vero eos et accusam
et justo duo dolores et ea rebum. Stet clita kasd gubergren, no sea
takimata sanctus est Lorem ipsum dolor sit amet. 

\subsubsection{Duis Autem}

Lorem ipsum dolor sit amet, consetetur sadipscing elitr, sed diam
nonumy eirmod tempor invidunt ut labore et dolore magna aliquyam erat,
sed diam voluptua. At vero eos et accusam et justo duo dolores et ea
rebum. Stet clita kasd gubergren, no sea takimata sanctus est Lorem
ipsum dolor sit amet. Lorem ipsum dolor sit amet, consetetur
sadipscing elitr, sed diam nonumy eirmod tempor invidunt ut labore et
dolore magna aliquyam erat, sed diam voluptua. At vero eos et accusam
et justo duo dolores et ea rebum. Stet clita kasd gubergren, no sea
takimata sanctus est Lorem ipsum dolor sit amet. Lorem ipsum dolor sit
amet, consetetur sadipscing elitr, sed diam nonumy eirmod tempor
invidunt ut labore et dolore magna aliquyam erat, sed diam
voluptua. At vero eos et accusam et justo duo dolores et ea
rebum. Stet clita kasd gubergren, no sea takimata sanctus est. Lorem
ipsum dolor sit amet.

\begin{figure}[tb]
 \centering % avoid the use of \begin{center}...\end{center} and use \centering instead (more compact)
 \includegraphics[width=\columnwidth]{paper-count-w-2015-new}
 \caption{A visualization of the 1990--2015 data from \autoref{tab:vis_papers}. The image is from \cite{Isenberg:2017:VMC} and is in the public domain.}
 \label{fig:sample}
\end{figure}

\subsubsection{Ejector Seat Reservation}

Duis autem~\cite{Lorensen:1987:MCA}\footnote{The algorithm behind
Marching Cubes \cite{Lorensen:1987:MCA} had already been
described by Wyvill et al. \cite{Wyvill:1986:DSS} a year
earlier.} vel eum iriure dolor in hendrerit
in vulputate velit esse molestie consequat,\footnote{Footnotes
appear at the bottom of the column.} vel illum dolore eu
feugiat nulla facilisis at vero eros et accumsan et iusto odio
dignissim qui blandit praesent luptatum zzril delenit augue duis
dolore te feugait nulla facilisi. Lorem ipsum dolor sit amet,
consectetuer adipiscing elit, sed diam nonummy nibh euismod tincidunt
ut laoreet dolore magna aliquam erat volutpat.


\paragraph{Confirmed Ejector Seat Reservation}

Ut wisi enim ad minim veniam, quis nostrud exerci tation ullamcorper
suscipit lobortis nisl ut aliquip ex ea commodo
consequat~\cite{Nielson:1991:TAD}. Duis autem vel eum iriure dolor in
hendrerit in vulputate velit esse molestie consequat, vel illum dolore
eu feugiat nulla facilisis at vero eros et accumsan et iusto odio
dignissim qui blandit praesent luptatum zzril delenit augue duis
dolore te feugait nulla facilisi.

\paragraph{Rejected Ejector Seat Reservation}

Ut wisi enim ad minim veniam, quis nostrud exerci tation ullamcorper
suscipit lobortis nisl ut aliquip ex ea commodo consequat. Duis autem
vel eum iriure dolor in hendrerit in vulputate velit esse molestie

\subsection{Vestibulum}

Vestibulum ut est libero. Suspendisse non libero id massa congue egestas nec at ligula. Donec nibh lorem, ornare et odio eu, cursus accumsan felis. Pellentesque habitant morbi tristique senectus et netus et malesuada fames ac turpis egestas. Donec dapibus quam vel eros mattis, id ornare dolor convallis. Donec at nisl sapien. Integer fringilla laoreet tempor. Fusce accumsan ante vel augue euismod, sit amet maximus turpis mattis. Nam accumsan vestibulum rhoncus. Aenean quis pellentesque augue. Suspendisse sed augue et velit consequat bibendum id nec est. Quisque erat purus, ullamcorper ut ex vel, dapibus dignissim erat.

Quisque sit amet orci quam. Lorem ipsum dolor sit amet, consectetur adipiscing elit. Aliquam pharetra, nunc non efficitur convallis, tellus purus iaculis lorem, nec ultricies dolor ligula in metus. Class aptent taciti sociosqu ad litora torquent per conubia nostra, per inceptos himenaeos. Aenean eu ex nulla. Morbi id ex interdum, scelerisque lorem nec, iaculis dui. Phasellus ultricies nunc vitae quam fringilla laoreet. Quisque sed dolor at sem vestibulum fringilla nec ac augue. Ut consequat, velit ac mattis ornare, eros arcu pellentesque erat, non ultricies libero metus nec mi. Sed eget elit sed quam malesuada viverra. Quisque ullamcorper, felis ut convallis fermentum, purus ligula varius ligula, sit amet tempor neque dui non neque. Donec vulputate ultricies tortor in mollis.

Integer sit amet dolor sit amet turpis ullamcorper varius. Cras volutpat bibendum scelerisque. Maecenas mauris dolor, gravida eu elit et, sodales consequat tortor. Integer id commodo elit. Pellentesque sollicitudin ex non nulla molestie eleifend. Mauris sagittis metus nec turpis imperdiet, vel ullamcorper nibh tincidunt. Sed semper tempus ex, ut aliquet erat hendrerit id. Maecenas sit amet dolor sollicitudin, luctus nunc sit amet, malesuada justo.

Mauris ut sapien non ipsum imperdiet sodales sit amet ac diam. Nulla vel convallis est. Etiam dapibus augue urna. Aenean enim leo, fermentum quis pulvinar at, ultrices quis enim. Sed placerat porta libero et feugiat. Phasellus ullamcorper, felis id porta sollicitudin, dolor dui venenatis augue, vel fringilla risus massa non risus. Maecenas ut nulla vitae ligula pharetra feugiat non eu ante. Donec quis neque quis lorem cursus pretium ac vulputate quam. Cras viverra tellus vitae sapien pretium laoreet. Pellentesque fringilla odio venenatis ex viverra, quis eleifend tortor ornare. Ut ut enim nunc. Vivamus id ligula nec est dignissim eleifend.

Nunc ac velit tellus. Donec et venenatis mauris. Lorem ipsum dolor sit amet, consectetur adipiscing elit. Ut vitae lectus vel ante mollis congue. Vestibulum at cursus velit. Curabitur in facilisis enim. Vestibulum eget dui aliquet risus laoreet laoreet. Phasellus et est id magna interdum venenatis. Donec luctus vehicula justo sed laoreet. Quisque tincidunt suscipit augue, in molestie sem accumsan sed.
\section{Conclusion}

Lorem ipsum dolor sit amet, consetetur sadipscing elitr, sed diam
nonumy eirmod tempor invidunt ut labore et dolore magna aliquyam erat,
sed diam voluptua. At vero eos et accusam et justo duo dolores et ea
rebum. Stet clita kasd gubergren, no sea takimata sanctus est Lorem
ipsum dolor sit amet. Lorem ipsum dolor sit amet, consetetur
sadipscing elitr, sed diam nonumy eirmod tempor invidunt ut labore et
dolore magna aliquyam erat, sed diam voluptua. At vero eos et accusam
et justo duo dolores et ea rebum. Stet clita kasd gubergren, no sea
takimata sanctus est Lorem ipsum dolor sit amet. Lorem ipsum dolor sit
amet, consetetur sadipscing elitr, sed diam nonumy eirmod tempor
invidunt ut labore et dolore magna aliquyam erat, sed diam
voluptua. At vero eos et accusam et justo duo dolores et ea
rebum.

